R2-GP: Variance-Calibrated Priors for Additive Gaussian Processes

We develop R2-GP, an R2D2-type prior for Gaussian process (GP) generalised additive models (GAMs) that calibrates explained variance ($R^2$) for Mat\'ern covariance kernels. The function variance for standard Mat\'ern kernels depends jointly on the effect magnitude and length-scale. As such, smooth and rough components with identical amplitudes contribute very different amounts of variation. With independent priors on component amplitudes, this variation results in variance overestimation, especially in higher dimensions. We overcome this by taking direct control over each component's expected contribution to prior explained variance. We do this by rescaling each component based on its length scale and observed inputs, and modelling each rescaled variance as a share of the function variance induced by a global $R^2$ prior. This allows R2-GP to scale well to many components. To also scale to large sample sizes, we extend R2-GP to Hilbert space approximation methods, a framework for kernels exploiting their spectral decompositions for fast and efficient inference. Our simulations and real-world case studies demonstrate superior generalisation and parameter recovery over independent variance priors.

==> tables/sparse/m32/parameter_recovery.tex <==
\begin{table*}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{2.5pt}
\caption{RMSE of the posterior mean relative to that under the R2-GP prior (sparse DGP, Mat\'ern $3/2$ kernel), from RMSEs averaged over 50 replications: a value above one is recovered worse than under R2-GP. The R2-GP rows give its RMSE itself, in italics. Columns give the number of additive components $D$. Only the leading components carry signal: the RMSE of $\alpha$ is taken separately across the active and the inactive components (true $\alpha_d = 0$), and that of $\rho$ across the active ones. Bold marks the lowest RMSE in each column within a length-scale. All models use the $N(\rho, 0.1)$ prior centred at the generating length-scale on the length-scales. Inputs are scaled to $[-1,1]$, so $\rho$ is relative to a unit half-range.}\label{tab:rmse-sparse-m32}
\begin{tabular}{ll *{20}{r}}
\toprule
 &  & \multicolumn{5}{c}{$\alpha$, active} & \multicolumn{5}{c}{$\alpha$, inactive} & \multicolumn{5}{c}{$\rho$} & \multicolumn{5}{c}{$\sigma$} \\
\cmidrule(lr){3-7} \cmidrule(lr){8-12} \cmidrule(lr){13-17} \cmidrule(lr){18-22}
$\rho$ & Prior & 5 & 10 & 30 & 50 & 100 & 5 & 10 & 30 & 50 & 100 & 5 & 10 & 30 & 50 & 100 & 5 & 10 & 30 & 50 & 100 \\
\midrule
0.3 & R2-GP & \textbf{\textit{0.087}} & \textbf{\textit{0.121}} & \textit{0.176} & \textit{0.207} & \textit{0.244} & --- & \textit{0.163} & \textit{0.109} & \textit{0.085} & \textit{0.060} & \textit{0.019} & \textit{0.016} & \textit{0.015} & \textit{0.012} & \textit{0.010} & \textit{0.056} & \textbf{\textit{0.066}} & \textbf{\textit{0.079}} & \textbf{\textit{0.106}} & \textbf{\textit{0.103}} \\
 & Normal & 1.61 & 1.14 & \textbf{0.93} & \textbf{0.66} & \textbf{0.27} & --- & 1.35 & 2.21 & 2.72 & 4.15 & 1.07 & 1.15 & 1.36 & 1.38 & 1.15 & \textbf{0.94} & 1.03 & 4.79 & 6.91 & 7.46 \\
 & NG & 1.56 & 1.34 & 1.11 & 0.94 & 0.70 & --- & 0.77 & 0.72 & 0.93 & 1.62 & 0.97 & 0.98 & 1.09 & 1.19 & 1.68 & 0.97 & 1.05 & 1.49 & 2.45 & 7.20 \\
 & RHS ($p_0{=}5$) & 1.70 & 1.51 & 1.24 & 1.17 & 1.10 & --- & \textbf{0.55} & \textbf{0.48} & \textbf{0.43} & \textbf{0.36} & \textbf{0.87} & \textbf{0.83} & \textbf{0.82} & \textbf{0.72} & \textbf{0.83} & 1.17 & 1.20 & 1.08 & 1.21 & 1.36 \\
\addlinespace
0.5 & R2-GP & \textbf{\textit{0.096}} & \textbf{\textit{0.116}} & \textit{0.187} & \textit{0.213} & \textit{0.235} & --- & \textit{0.163} & \textit{0.100} & \textit{0.081} & \textit{0.064} & \textit{0.012} & \textit{0.011} & \textit{0.009} & \textit{0.007} & \textit{0.008} & \textbf{\textit{0.065}} & \textit{0.067} & \textbf{\textit{0.066}} & \textbf{\textit{0.079}} & \textbf{\textit{0.123}} \\
 & Normal & 1.78 & 1.43 & \textbf{0.79} & \textbf{0.70} & \textbf{0.38} & --- & 1.36 & 2.45 & 3.35 & 4.13 & 0.98 & 0.94 & 1.16 & 1.28 & 1.25 & 1.02 & 1.00 & 3.54 & 7.64 & 6.29 \\
 & NG & 1.60 & 1.44 & 1.14 & 1.06 & 0.73 & --- & 0.75 & 0.63 & 0.63 & 1.54 & 0.94 & 0.90 & 0.93 & 1.05 & 1.40 & 1.02 & \textbf{0.99} & 1.30 & 1.48 & 5.17 \\
 & RHS ($p_0{=}5$) & 1.68 & 1.55 & 1.20 & 1.13 & 1.07 & --- & \textbf{0.55} & \textbf{0.49} & \textbf{0.43} & \textbf{0.42} & \textbf{0.89} & \textbf{0.80} & \textbf{0.78} & \textbf{0.79} & \textbf{0.89} & 1.08 & 1.13 & 1.10 & 1.42 & 1.02 \\
\addlinespace
0.7 & R2-GP & \textbf{\textit{0.097}} & \textbf{\textit{0.117}} & \textit{0.187} & \textit{0.213} & \textit{0.235} & --- & \textit{0.162} & \textit{0.099} & \textit{0.079} & \textit{0.063} & \textit{0.007} & \textit{0.007} & \textit{0.006} & \textit{0.005} & \textit{0.005} & \textit{0.063} & \textit{0.066} & \textbf{\textit{0.054}} & \textbf{\textit{0.068}} & \textit{0.114} \\
 & Normal & 1.82 & 1.53 & \textbf{0.86} & \textbf{0.81} & \textbf{0.48} & --- & 1.45 & 2.57 & 3.67 & 4.49 & 0.90 & 0.95 & 1.12 & 1.28 & 1.79 & \textbf{0.97} & 0.99 & 3.30 & 6.83 & 6.83 \\
 & NG & 1.59 & 1.45 & 1.15 & 1.11 & 0.74 & --- & 0.78 & 0.60 & 0.55 & 1.49 & 0.87 & 0.91 & 1.00 & 0.98 & 1.47 & 1.00 & \textbf{0.97} & 1.13 & 1.24 & 4.51 \\
 & RHS ($p_0{=}5$) & 1.66 & 1.53 & 1.18 & 1.11 & 1.06 & --- & \textbf{0.55} & \textbf{0.49} & \textbf{0.44} & \textbf{0.43} & \textbf{0.84} & \textbf{0.82} & \textbf{0.83} & \textbf{0.83} & \textbf{0.88} & 1.09 & 1.11 & \textbf{1.00} & 1.37 & \textbf{0.96} \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/sparse/m52/parameter_recovery.tex <==
\begin{table*}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{2.5pt}
\caption{RMSE of the posterior mean relative to that under the R2-GP prior (sparse DGP, Mat\'ern $5/2$ kernel), from RMSEs averaged over 50 replications: a value above one is recovered worse than under R2-GP. The R2-GP rows give its RMSE itself, in italics. Columns give the number of additive components $D$. Only the leading components carry signal: the RMSE of $\alpha$ is taken separately across the active and the inactive components (true $\alpha_d = 0$), and that of $\rho$ across the active ones. Bold marks the lowest RMSE in each column within a length-scale. All models use the $N(\rho, 0.1)$ prior centred at the generating length-scale on the length-scales. Inputs are scaled to $[-1,1]$, so $\rho$ is relative to a unit half-range.}\label{tab:rmse-sparse-m52}
\begin{tabular}{ll *{20}{r}}
\toprule
 &  & \multicolumn{5}{c}{$\alpha$, active} & \multicolumn{5}{c}{$\alpha$, inactive} & \multicolumn{5}{c}{$\rho$} & \multicolumn{5}{c}{$\sigma$} \\
\cmidrule(lr){3-7} \cmidrule(lr){8-12} \cmidrule(lr){13-17} \cmidrule(lr){18-22}
$\rho$ & Prior & 5 & 10 & 30 & 50 & 100 & 5 & 10 & 30 & 50 & 100 & 5 & 10 & 30 & 50 & 100 & 5 & 10 & 30 & 50 & 100 \\
\midrule
0.3 & R2-GP & \textbf{\textit{0.100}} & \textbf{\textit{0.114}} & \textit{0.183} & \textit{0.201} & \textit{0.240} & --- & \textit{0.162} & \textit{0.103} & \textit{0.087} & \textit{0.062} & \textit{0.020} & \textit{0.018} & \textit{0.015} & \textit{0.014} & \textit{0.011} & \textbf{\textit{0.067}} & \textbf{\textit{0.070}} & \textbf{\textit{0.069}} & \textbf{\textit{0.085}} & \textbf{\textit{0.124}} \\
 & Normal & 1.57 & 1.33 & \textbf{0.84} & \textbf{0.79} & \textbf{0.30} & --- & 1.32 & 2.31 & 2.76 & 4.04 & 1.01 & 1.17 & 1.26 & 1.41 & 1.05 & \textbf{1.00} & 1.12 & 4.31 & 8.10 & 6.19 \\
 & NG & 1.54 & 1.39 & 1.12 & 0.99 & 0.69 & --- & 0.77 & 0.67 & 0.83 & 1.57 & 0.92 & 1.01 & 0.98 & 1.33 & 1.77 & 1.02 & 1.05 & 1.43 & 2.47 & 5.98 \\
 & RHS ($p_0{=}5$) & 1.62 & 1.51 & 1.22 & 1.16 & 1.09 & --- & \textbf{0.57} & \textbf{0.46} & \textbf{0.44} & \textbf{0.40} & \textbf{0.88} & \textbf{0.91} & \textbf{0.78} & \textbf{0.85} & \textbf{0.80} & 1.09 & 1.08 & 1.25 & 1.21 & 1.03 \\
\addlinespace
0.5 & R2-GP & \textbf{\textit{0.099}} & \textbf{\textit{0.125}} & \textit{0.186} & \textit{0.195} & \textit{0.237} & --- & \textit{0.158} & \textit{0.098} & \textit{0.089} & \textit{0.061} & \textit{0.013} & \textit{0.012} & \textit{0.010} & \textit{0.010} & \textit{0.008} & \textbf{\textit{0.055}} & \textbf{\textit{0.060}} & \textbf{\textit{0.064}} & \textit{0.077} & \textit{0.114} \\
 & Normal & 1.83 & 1.28 & \textbf{0.84} & \textbf{0.99} & \textbf{0.39} & --- & 1.46 & 2.55 & 3.13 & 4.42 & 0.94 & 1.02 & 1.17 & 1.32 & 1.43 & 1.02 & 1.06 & 2.68 & 6.89 & 6.87 \\
 & NG & 1.60 & 1.34 & 1.15 & 1.16 & 0.72 & --- & 0.77 & 0.52 & 0.62 & 1.59 & 0.90 & 0.90 & 0.93 & 1.08 & 1.48 & 1.01 & 1.03 & 1.19 & 1.40 & 5.28 \\
 & RHS ($p_0{=}5$) & 1.68 & 1.47 & 1.19 & 1.11 & 1.07 & --- & \textbf{0.54} & \textbf{0.46} & \textbf{0.51} & \textbf{0.42} & \textbf{0.85} & \textbf{0.81} & \textbf{0.74} & \textbf{0.87} & \textbf{0.85} & 1.04 & 1.09 & 1.23 & \textbf{0.97} & \textbf{0.99} \\
\addlinespace
0.7 & R2-GP & \textbf{\textit{0.100}} & \textbf{\textit{0.126}} & \textit{0.188} & \textbf{\textit{0.197}} & \textit{0.234} & --- & \textit{0.156} & \textit{0.096} & \textit{0.087} & \textit{0.062} & \textit{0.009} & \textit{0.008} & \textit{0.007} & \textit{0.007} & \textit{0.006} & \textbf{\textit{0.053}} & \textbf{\textit{0.061}} & \textbf{\textit{0.063}} & \textit{0.074} & \textit{0.102} \\
 & Normal & 1.92 & 1.34 & \textbf{0.92} & 1.05 & \textbf{0.55} & --- & 1.56 & 2.76 & 3.36 & 4.74 & 0.90 & 0.94 & 1.06 & 0.94 & 2.26 & 1.01 & \textbf{1.00} & 2.07 & 4.93 & 7.88 \\
 & NG & 1.62 & 1.32 & 1.16 & 1.20 & 0.80 & --- & 0.80 & 0.52 & 0.56 & 1.27 & 0.89 & 0.89 & 0.92 & 0.87 & 1.16 & \textbf{1.00} & 1.01 & 1.17 & 1.15 & 3.79 \\
 & RHS ($p_0{=}5$) & 1.72 & 1.45 & 1.17 & 1.10 & 1.04 & --- & \textbf{0.55} & \textbf{0.47} & \textbf{0.51} & \textbf{0.44} & \textbf{0.86} & \textbf{0.83} & \textbf{0.76} & \textbf{0.81} & \textbf{0.86} & 1.01 & 1.05 & 1.20 & \textbf{0.92} & \textbf{0.98} \\
\bottomrule
\end{tabular}
\end{table*}


==> tables/sparse/se/parameter_recovery.tex <==
\begin{table*}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{2.5pt}
\caption{RMSE of the posterior mean relative to that under the R2-GP prior (sparse DGP, squared exponential kernel), from RMSEs averaged over 50 replications: a value above one is recovered worse than under R2-GP. The R2-GP rows give its RMSE itself, in italics. Columns give the number of additive components $D$. Only the leading components carry signal: the RMSE of $\alpha$ is taken separately across the active and the inactive components (true $\alpha_d = 0$), and that of $\rho$ across the active ones. Bold marks the lowest RMSE in each column within a length-scale. All models use the $N(\rho, 0.1)$ prior centred at the generating length-scale on the length-scales. Inputs are scaled to $[-1,1]$, so $\rho$ is relative to a unit half-range.}\label{tab:rmse-sparse-se}
\begin{tabular}{ll *{20}{r}}
\toprule
 &  & \multicolumn{5}{c}{$\alpha$, active} & \multicolumn{5}{c}{$\alpha$, inactive} & \multicolumn{5}{c}{$\rho$} & \multicolumn{5}{c}{$\sigma$} \\
\cmidrule(lr){3-7} \cmidrule(lr){8-12} \cmidrule(lr){13-17} \cmidrule(lr){18-22}
$\rho$ & Prior & 5 & 10 & 30 & 50 & 100 & 5 & 10 & 30 & 50 & 100 & 5 & 10 & 30 & 50 & 100 & 5 & 10 & 30 & 50 & 100 \\
\midrule
0.3 & R2-GP & \textbf{\textit{0.097}} & \textbf{\textit{0.118}} & \textit{0.179} & \textit{0.203} & \textit{0.242} & --- & \textit{0.158} & \textit{0.103} & \textit{0.086} & \textit{0.060} & \textit{0.022} & \textit{0.022} & \textit{0.017} & \textit{0.016} & \textit{0.013} & \textit{0.053} & \textit{0.082} & \textbf{\textit{0.084}} & \textbf{\textit{0.077}} & \textbf{\textit{0.102}} \\
 & Normal & 1.57 & 1.30 & \textbf{0.95} & \textbf{0.80} & \textbf{0.35} & --- & 1.40 & 2.34 & 2.98 & 4.35 & 1.06 & 1.17 & 1.39 & 1.42 & 0.95 & \textbf{0.98} & \textbf{0.93} & 2.66 & 7.94 & 7.56 \\
 & NG & 1.52 & 1.39 & 1.21 & 1.01 & 0.72 & --- & 0.74 & 0.56 & 0.70 & 1.65 & 0.93 & 1.00 & 1.07 & 1.18 & 1.67 & 1.00 & 1.05 & 1.24 & 1.97 & 6.88 \\
 & RHS ($p_0{=}5$) & 1.64 & 1.49 & 1.23 & 1.14 & 1.08 & --- & \textbf{0.54} & \textbf{0.47} & \textbf{0.44} & \textbf{0.39} & \textbf{0.88} & \textbf{0.87} & \textbf{0.82} & \textbf{0.78} & \textbf{0.83} & 1.11 & 1.15 & 1.18 & 1.23 & 1.15 \\
\addlinespace
0.5 & R2-GP & \textbf{\textit{0.092}} & \textbf{\textit{0.112}} & \textbf{\textit{0.180}} & \textit{0.205} & \textit{0.243} & --- & \textit{0.163} & \textit{0.103} & \textit{0.083} & \textit{0.058} & \textit{0.016} & \textit{0.014} & \textit{0.012} & \textit{0.011} & \textit{0.008} & \textit{0.053} & \textbf{\textit{0.067}} & \textbf{\textit{0.073}} & \textbf{\textit{0.075}} & \textbf{\textit{0.081}} \\
 & Normal & 1.96 & 1.64 & \textbf{1.00} & \textbf{0.90} & \textbf{0.52} & --- & 1.49 & 2.60 & 3.55 & 5.09 & 0.99 & 1.02 & 1.11 & 1.16 & 2.08 & \textbf{0.97} & 1.03 & 2.03 & 4.92 & 9.85 \\
 & NG & 1.65 & 1.41 & 1.17 & 1.13 & 0.77 & --- & 0.82 & 0.62 & 0.48 & 1.44 & 0.92 & 0.91 & 0.92 & 0.95 & 1.70 & 1.00 & 1.04 & \textbf{1.00} & 1.04 & 5.30 \\
 & RHS ($p_0{=}5$) & 1.76 & 1.50 & 1.17 & 1.11 & 1.06 & --- & \textbf{0.58} & \textbf{0.52} & \textbf{0.46} & \textbf{0.42} & \textbf{0.87} & \textbf{0.81} & \textbf{0.83} & \textbf{0.81} & \textbf{0.92} & 1.07 & 1.11 & 1.01 & 1.02 & 1.04 \\
\addlinespace
0.7 & R2-GP & \textbf{\textit{0.095}} & \textbf{\textit{0.118}} & \textbf{\textit{0.183}} & \textit{0.208} & \textit{0.243} & --- & \textit{0.160} & \textit{0.100} & \textit{0.080} & \textit{0.057} & \textit{0.011} & \textit{0.010} & \textit{0.009} & \textit{0.008} & \textit{0.006} & \textit{0.053} & \textbf{\textit{0.066}} & \textit{0.069} & \textit{0.069} & \textit{0.074} \\
 & Normal & 2.07 & 1.64 & 1.07 & \textbf{0.97} & \textbf{0.69} & --- & 1.67 & 2.89 & 3.90 & 5.74 & 0.95 & 0.98 & 1.05 & 1.04 & 2.52 & \textbf{0.98} & \textbf{1.00} & 1.64 & 3.56 & 10.69 \\
 & NG & 1.70 & 1.34 & 1.18 & 1.18 & 0.94 & --- & 0.85 & 0.60 & \textbf{0.46} & 0.95 & 0.91 & 0.91 & 0.89 & 0.93 & 1.36 & 1.00 & 1.01 & 1.02 & \textbf{0.91} & 2.52 \\
 & RHS ($p_0{=}5$) & 1.79 & 1.47 & 1.14 & 1.09 & 1.05 & --- & \textbf{0.59} & \textbf{0.53} & 0.47 & \textbf{0.44} & \textbf{0.86} & \textbf{0.80} & \textbf{0.88} & \textbf{0.81} & \textbf{0.89} & 1.05 & 1.11 & \textbf{0.97} & 0.98 & \textbf{0.95} \\
\bottomrule
\end{tabular}
\end{table*}

